Supernova Feedback in Molecular Clouds: Global Evolution and Dynamics

We use magnetohydrodynamical simulations of converging warm neutral medium flows to analyse the formation and global evolution of magnetised and turbulent molecular clouds subject to supernova feedback from massive stars. We show that supernova feedback alone fails to disrupt entire, gravitationally bound, molecular clouds, but is able to disperse small--sized (~10 pc) regions on timescales of less than 1 Myr. Efficient radiative cooling of the supernova remnant as well as strong compression of the surrounding gas result in non-persistent energy and momentum input from the supernovae. However, if the time between subsequent supernovae is short and they are clustered, large hot bubbles form that disperse larger regions of the parental cloud. On longer timescales, supernova feedback increases the amount of gas with moderate temperatures (T~300-3000 K). Despite its inability to disrupt molecular clouds, supernova feedback leaves a strong imprint on the star formation process. We find an overall reduction of the star formation efficiency by a factor of 2 and of the star formation rate by roughly factors of 2-4.

==> journals.tex <==
%% journal abbreviations (from aastex.cls)

\def\jnl@style#1{{\rmfamily#1}}%
\def\jref@jnl#1{{\jnl@style#1}}%

\newcommand\aj{\jref@jnl{AJ}}%
          % Astronomical Journal
\newcommand\araa{\jref@jnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\jref@jnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\jref@jnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\jref@jnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\jref@jnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\jref@jnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\jref@jnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\jref@jnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\jref@jnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\jref@jnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\jref@jnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\jrasc{\jref@jnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\jref@jnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\nar{\jref@nl{NAR}}
	  %New Astronomy Reviews
\newcommand\mnras{\jref@jnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\pra{\jref@jnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\jref@jnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\jref@jnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\jref@jnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\jref@jnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\jref@jnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasp{\jref@jnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\jref@jnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\jref@jnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\skytel{\jref@jnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\jref@jnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\jref@jnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\jref@jnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\jref@jnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand{\znat}{Z. Naturforsch}
          % Zeitschrift fuer Naturforschung
\newcommand\nat{\jref@jnl{Nature}}%
          % Nature
\newcommand\iaucirc{\jref@jnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\jref@jnl{Astrophys.~Lett.}}%
          % Astrophysics Letters
\newcommand\apspr{\jref@jnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\jref@jnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\jref@jnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\jref@jnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\jref@jnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\jref@jnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jcop{\jref@jnl{J.~Comp.~Phys.}}%
          % Journal of Computational Physics
\newcommand\jgr{\jref@jnl{J.~Geophys.~Res.}}%
          % Journal of Geophysics Research
\newcommand{\jkas}{Journ. Korean. Astron. Soc.}
          % Journal of the Korean Astronomical Society
\newcommand\jqsrt{\jref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\jref@jnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\jref@jnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\jref@jnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\jref@jnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\jref@jnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\jref@jnl{Proc.~SPIE}}%
          % Proceedings of the SPIE

